Continual Learning in Medical Image Analysis: A Comprehensive Review of Recent Advancements and Future Prospects

Medical imaging analysis has witnessed remarkable advancements even surpassing human-level performance in recent years, driven by the rapid development of advanced deep-learning algorithms. However, when the inference dataset slightly differs from what the model has seen during one-time training, the model performance is greatly compromised. The situation requires restarting the training process using both the old and the new data which is computationally costly, does not align with the human learning process, and imposes storage constraints and privacy concerns. Alternatively, continual learning has emerged as a crucial approach for developing unified and sustainable deep models to deal with new classes, tasks, and the drifting nature of data in non-stationary environments for various application areas. Continual learning techniques enable models to adapt and accumulate knowledge over time, which is essential for maintaining performance on evolving datasets and novel tasks. This systematic review paper provides a comprehensive overview of the state-of-the-art in continual learning techniques applied to medical imaging analysis. We present an extensive survey of existing research, covering topics including catastrophic forgetting, data drifts, stability, and plasticity requirements. Further, an in-depth discussion of key components of a continual learning framework such as continual learning scenarios, techniques, evaluation schemes, and metrics is provided. Continual learning techniques encompass various categories, including rehearsal, regularization, architectural, and hybrid strategies. We assess the popularity and applicability of continual learning categories in various medical sub-fields like radiology and histopathology...

==> content/keywords.tex <==

Continual Learning\sep
Drift\sep
Domain Shift\sep
Concept Drift\sep
Medical Image Analysis\sep
Histopathology\sep
Radiology

==> content/sections/sec-snigle/background.tex <==
\section{Background}
\label{sec:background}


% Medical data drifts in non-stationary environment
\subsection{Medical data drifts}
\label{sec:medical-data-drifts}
In clinical practices, the data distribution evolves over time, reflecting the dynamic nature of the healthcare environment \cite{sahiner2023data, LACS, MORE}. Inconsistencies in data collection procedures across different healthcare settings or institutions contribute to data drift. Also, the introduction of new medical imaging devices, diagnostic tools, and data acquisition techniques leads to a shift in the technological landscape \cite{derakhshani2022lifelonger, LACS}. Moreover, the advancement in medical research and the discovery of new diseases/treatment methods raise the understanding of healthcare. This new knowledge can influence the characteristics of medical data that cause shifts in the underlying distribution \cite{LACS, MORE}. Also, data sources can have their dynamics and therefore are inherently non-constant. For instance, cardiac CT images are captured under time-varying factors such as breathing and heart rates. Non-homogeneous data is another challenge, as individual health differences among patients can vary over time due to factors like genetics, age, occupation, and lifestyle \cite{LACS, BER}.
Additionally, variations in sample preparation or pre-processing methods contribute to distinctions among imaging datasets. In digital histopathology, differences in staining policies across labs introduce undesired stain variances in whole-slide images \cite{AIPath, AM}. The imaging solution may also influence the final digital visualization throughout the entire learning process over time. Nonlinear augmentation of computed radiography occurs at various degrees due to the differing physical and chemical properties of contrast mediums from different brands. Variables like sensor signal-to-noise ratio (SNR), customized parameter settings in imaging software, and storage-friendly distortions can all impact the quality of the resultant image. For instance, in digital histopathology, billion-pixel whole slide images (WSI) at a fixed magnification have seen variations in storage size, ranging from megabytes to gigabytes per image over the years, consequently enhancing the dataset quality in terms of micron-per-pixel (MPP) for continual learning tasks \cite{AIPath}.

The medical data drifts can have significant implications for the performance and reliability of machine learning and deep learning models \cite{BER}. Traditional machine learning often relies heavily on static data and feature engineering, where human experts manually select the relevant features. In the case of data drift, these handcrafted features may become less informative, and the model may struggle to adapt to new patterns \cite{BAYRAM2022108632}. More specifically, for both machine learning and deep learning, this issue is particularly prevalent in dynamic and non-stationary environments, where the statistical properties of the data evolve. Understanding the sources of drift, such as inconsistencies in data collection and technological advancements, is crucial for developing robust models \cite{BER}. Proactive strategies, including regular model updates and continuous monitoring, are essential to ensure that machine learning models remain effective and reliable in navigating the evolving healthcare landscape. By addressing medical data drift and developing machine learning models that can adapt to the ever-changing nature of clinical data, ultimately enhancing patient care and outcomes.


% Catastrophic forgetting
\subsection{Catastrophic forgetting}
\label{sec:catastrophic-forgetting}
Throughout a lifetime, a human brain continuously acquires knowledge, and learning new concepts or tasks has no detrimental effect on previously learned ones. Instead, learning several closely related concepts even boosts the learning of all associated ones. In contrast, artificial neural networks, although inspired by the human brain, often suffer from `catastrophic forgetting', a tendency to overwrite or forget the knowledge acquired in the past upon learning new concepts~\cite{mccloskey1989catastrophic,ratcliff1990connectionist}. This can be attributed to the fact that the model entirely optimizes for the given dataset. In other words, a model with optimized weights for a task \textbf{T1}, when trained on a new task \textbf{T2}, will freely optimize the existing weights to meet the objectives in task \textbf{T2}, which may now no longer be optimal for the previous task \textbf{T1}. This can be a significant challenge, especially in scenarios where an AI system is expected to learn and adapt to a stream of tasks or datasets over time. Catastrophic forgetting in neural networks is an interesting phenomenon that has attracted lots of attention in recent research~\cite{goodfellow2013empirical,KUMARI2024117100}.


% Continual learning overview
\subsection{Continual learning overview}
\label{sec:essence-of-cl}
A naive solution to deal with catastrophic forgetting can be retraining the model collectively on old and new data from scratch each time new data with drifted distribution or classes are encountered \cite{lee2020clinical}. This process mostly gives the desired classification or segmentation performance; however, it causes an intense burden on computing and storage requirements and, hence, is impractical for deployment. Additionally, the retraining process requires storing the past data and thus causes privacy violations, which can be a major bottleneck of such a strategy in healthcare applications. 

Alternately, CL, also termed as `continuously learning', `incremental learning', `sequential learning' or `lifelong learning', has emerged as a promising solution in various fields to deal with the catastrophic forgetting issue \cite{de2021continual,mai2022online}. 
%%%%%In dynamic real-world environments, where data distributions may change or new tasks emerge, a continuous adaptation of the environment is crucial for AI systems to be robust, reliable, and efficient. 
It helps in efficiently leveraging existing knowledge and incorporating new information without the need for extensive retraining. The primary goal of CL is to develop techniques and strategies that allow a neural network to learn new tasks while retaining knowledge of previous tasks. In other words, it aims to enable the network to continually adapt to new information without completely erasing or degrading its performance on earlier tasks. Overall, CL helps to address the issue of catastrophic forgetting and minimizes the need for additional resources to store historical data. 
CL offers a range of strategies and methods, such as regularization (constraining weight update to avoid forgetting learnt concepts), rehearsal (partially using some form of old data to replay with current data), and architectural modifications (reserving or partitioning network for different tasks), to help neural networks remember and consolidate knowledge from past tasks. These strategies help prevent or reduce catastrophic forgetting and improve the generalization ability of the model.


% Continual learning pipeline
%===========================================
\begin{figure}[!ht]
    \centering
    \includegraphics[width=.48\textwidth]{content/figures/drawn/cl-pipeline.pdf}
    \caption{A coarse level flowchart for designing a CL pipeline}
    \label{fig:pipeline}
\end{figure}
%===========================================
\subsection{Continual learning pipeline}
\label{sec:cl-pipeline}
The design of a CL pipeline is illustrated in ~\refx{fig:pipeline} which provides an overview of the key components and stages involved in the construction of the CL pipeline. Given a problem statement, first, we need to identify which CL scenarios it falls under, i.e., whether there is a possibility of domain shifts in future data, inclusion of new classes, or the end application, i.e., the task itself may change. For example, if we want to develop a breast cancer classification model to be able to work on the H\&E dataset from different centers then the datasets across centers may have drift and hence fall into the domain incremental scenario of CL. Detailed information about CL scenarios is provided in \refx{sec:CLscenario}. Once we have identified the CL scenario, training, and testing, datasets need to be prepared to mimic a continual stream of datasets arriving one after another. The sequence of datasets is frequently referred to as tasks or episodes in literature. We also use these two terms interchangeably in this manuscript. 
%%%%Since the term `task' is also used for end application and thus may be challenging to get the true interpretation of the term, hence, we use the term `episode' to refer to the sequence of datasets in a CL pipeline. 
For each episode, separate training and testing data is prepared; thus, the pipeline requires four train-test pairs to develop and evaluate a CL model for four sequential datasets. Once the datasets are ready, a CL strategy suitable to the task at hand is identified and deployed in any off-the-shelf deep classification or segmentation model. There are various CL strategies, some offering privacy-preserved learning, while some offer better performance but at the cost of more resources, storage, and privacy violations as they store some past data. Typically, the model is trained on the first training episode and evaluated on testing data from all the episodes. After this, the training shifts to the next episode, where the inclusion of partial training data from the previous episode is possible. Here, updating the model with new training data, the evaluation is again done on all the testing data, and the process repeats until the last episode. Application-specific performance metrics (e.g., accuracy, dice similarity coefficient, etc.) computed on testing data of each episode are observed and analyzed over the sequence. Then, we can compute various metrics on top of it to quantify forgetting and forward transfer. Lastly, the CL framework is evaluated against state-of-the-art works and non-CL methods offering upper and lower bounds of performance. Joint or cumulative training gives the highest average performance, whereas naively finetuning on the current episode gives the lowest performance~\cite{kaustaban2022characterizing,lenga2020continual}.

% Application of continual learning
%===========================================
\begin{figure}[!ht]
\centering
% \includegraphics[scale=0.45]{content/figures/drawn/chart_segmentation.pdf}
\includegraphics[width=.48\textwidth]{content/figures/charts/chart_segmentation.pdf}
\caption{Ratio of CL-based research for downstream applications}
\label{fig:pieChartSegmentation}
\end{figure}
%===========================================
%===========================================
\begin{figure}[!ht]
\centering
% \includegraphics[scale=0.45]{content/figures/drawn/chart_papers_over_year.pdf}
\includegraphics[width=.48\textwidth]{content/figures/charts/chart_papers_over_year.pdf}
\caption{CL-based research contributions over the year}
\label{fig:pieChartPaperOverYear}
\end{figure}
%===========================================
\subsection{Application of continual learning}\label{sec:application-of-cl}

CL has numerous applications across various domains due to its ability to mitigate catastrophic forgetting. The efficiency and robustness of CL in real-time scenarios derive from its ability to adapt, reduce computational overhead, and address the challenges of dynamic data. This makes it a valuable approach for applications where time constraints, adaptability, and efficiency are of great importance. In the medical domain, CL has been widely explored for various segmentation and classification applications (\refx{fig:pieChartSegmentation}) and continuously exhibited its merits over static models as reflected by the increasing number of research contributions over the year (\refx{fig:pieChartPaperOverYear}).
CL can improve the diagnosis and decision-making ability in a resource-constrained environment. Further, it is beneficial in real-time monitoring of patients, telemedicine, and maintaining a dynamic knowledge base. This section presents the most prominent applications of CL in medical settings in terms of the number of publications.

%%%\textbf{Applications of Domain incremental settings: }
\textbf{Radiology and imaging}:
Radiological imaging techniques are continually advancing, requiring models to adapt to new technologies and methodologies. For CT, research has investigated the impact of scanners and reconstruction parameters on both machine learning predictions and human annotations. The findings indicate that the variability introduced by different scanners has a detrimental effect on radiomics \cite{radio1,radio2}  and other imaging features. Therefore, it is imperative to take into account this scanner variability when developing machine learning models. CL facilitates the dynamic adjustment of models to evolving imaging techniques, ensuring accurate interpretations ~\cite{radio3} ~\cite{radio4}. \refx{tab:classificationCL} and \refx{tab:segmentationCL} present the selected works for CL-based classification and segmentation in the medical domain.

\textbf{Disease progression modeling}: CL is crucial in tracking the progression of diseases such as Alzheimer's Disease (AD). Models must adapt to new patient data over time, incorporating the latest diagnostic criteria and treatment strategies~\cite{li2020continual}. Recent work was proposed for modeling AD progression in a CL manner that respects the longitudinal data sets coming in sequence and ensures equal prediction accuracy for future visits~\cite{Alz}.

%%%%\textbf{Applications of class incremental settings:}
\textbf{Drug discovery}: CL can accelerate drug discovery by continuously integrating newly discovered chemical compounds, pharmacological data, and clinical trial results to predict drug interactions and efficacy. A recent work presented a CL-based model called Multi-Scale Temporal Convolutional Networks-based AntiBacterial Peptide prediction (MSTCN-ABPpred). This model is designed for the classification and discovery of antibacterial peptides (ABPs). While MSTCN-ABPpred can dynamically adapt and retrain based on predicted ABPs and non-ABPs within protein sequences, it does have limitations in terms of providing information about the identified ABPs' targets, haemotoxicity, cytotoxicity, and minimum inhibitory concentration (MIC) against various bacteria ~\cite{DD}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


==> content/sections/sec-snigle/cl-scenarios.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Continual learning scenarios}
\label{sec:CLscenario}
Depending upon what kind of change in the sequence of data is expected, the existing CL scenarios can be broadly categorized into five categories, viz., (a) data-incremental, (b) class-incremental, (c) task-incremental, (d) domain-incremental, and (e) hybrid. \refx{fig:pieChartCLscenarios} shows the percentages of the above-mentioned incremental CL scenarios exploited in recent years. The statistics reflect that domain-incremental is highly explored with a 51.9\% ratio out of five major settings, followed by the class-incremental settings having 26.9\% works and data-incremental being the least challenging and rarely explored for different medical image analysis applications.

%===========================================
\begin{figure}[!ht]
\centering
% \includegraphics[scale=0.45]{content/figures/drawn/chart_cl_scenarios.pdf}
\includegraphics[width=.48\textwidth]{content/figures/charts/chart_cl_scenarios.pdf}
\caption{Ratio of CL-based works for different incremental scenarios}
\label{fig:pieChartCLscenarios}
\end{figure}
%===========================================

% ======= Instance incremental scenarios =======
\subsection{Instance incremental scenarios}
\label{sec:data-incremental-scenarios}
\input{content/tables/data-incremental-detail}

Instance Incremental Scenario (IIS), also termed as data incremental scenario, involves the continuous learning process where the model keeps adapting to incoming data streams that come from the same data distribution. This scenario doesn't involve dealing with entirely new categories or significant changes in data patterns, making it generally the least challenging among all other CL scenarios. In the medical domain, especially digital pathology, a common practice is for expert pathologists to annotate a dataset in multiple stages or batches~\cite{kaustaban2022characterizing}. Each of these annotation batches can be thought of as representing samples from the same underlying data distribution, ensuring some consistency in the data source across different batches. Thus, IIS scenarios deal with the condition where the samples of a dataset are sequentially made available. Owning to its simplicity, this category is not very popular. Only a few classification applications are explored in this scenario, as mentioned in \refx{tab:dataIncrementalDetailTable}. For example, in the breast cancer classification application, \citet{chen2022breast} set up IIS on the BreakHis~\cite{spanhol2015dataset} dataset. More and more samples from each of the malignant and benign classes are added over the subsequent episodes. 
\citet{ravishankar2019feature} try to exhibit a scenario for pneumothorax detection in a hospital where data arrives in an incremental fashion. They sequentially fed 2000 samples in 4 subsequent episodes from an X-ray dataset for Pneumothorax identification consisting of a total of 8000 samples.  


\input{content/tables/class-incremental-detail}

\subsection{Class incremental scenarios}
\label{sec:cl-scenarios}

%%% from a paper: It refers to continuously extend an existing model to unseen classes with new streams of data. Since the knowledge to learn from each batch of unseen classes is largely non-overlapping, this scenario is expected to be the hardest among CL scenarios. For example, adding new tissue types in a tumor classification model or adding new cell types into a cell detection model for AI-assisted diagnosis.


Class Incremental Scenario (CIS) refers to a situation where the aim is to adapt the model to accommodate novel classes from new data streams. Given that each batch of these unseen classes offers knowledge that largely differs from the previous batches, this scenario is anticipated to be the most challenging among continual learning scenarios. An instance of this challenge is incorporating new types of tissues into a tumor classification model or introducing novel cell types into a model designed for AI-assisted diagnosis in cell detection. In this scenario, there is only one incremental task that gets additions of new classes in subsequent episodes. Some works assume mutually exclusive classes, whereas some overlapping classes.


Multi-class datasets with more than 5-6 classes are mainly considered to create a class incremental scenario. There can be an equal or variable number of classes across the episodes. \citet{chen2022breast} propose a breast cancer classification model where they iteratively include malignant and benign classes with one sub-class from each category. This scenario is very popular for segmentation applications where the model may be demanded to segment more and more classes over time. 
An exhaustive list of class incremental scenarios explored in literature is provided via \refx{tab:classIncrementalDetailTable}. References, along with detailed segmentation or classification applications, are tabulated.  



\input{content/tables/task-incremental-detail}
\input{content/sections/cl-scenarios/task-incremental}


\input{content/tables/domain-shift-detail}
\input{content/sections/cl-scenarios/domain-incremental}


\input{content/tables/hybrid-detail}
\input{content/sections/cl-scenarios/simulated-or-hybrid-settings}



==> content/sections/sec-snigle/introduction.tex <==
\section{Introduction}
\label{sec:introduction}


In the evolving field of medical image analysis, the dynamic nature of healthcare data poses a critical challenge for the generalizability of the machine learning/deep learning models to new data/domains \cite{miotto, 9363915}. The data-driven approaches have challenges due to the limited availability and accessibility of sufficiently large and diverse medical data for training \cite{miotto, Hao, 9363915, JOC1, JOC2}. Additionally, the source variability, scanner manufacturer, imaging protocol, and diverse population groups make the medical data heterogeneous, this adds a bias and discrepancies between training and testing datasets, thus leading to performance degradation \cite{Luca, 9363915}. In order to handle the model generalizability issues, domain adaptation methods become popular and aim to transfer knowledge from one domain to other unseen data sources or domains \cite{jeff01, Jeff02, Hao, CW, becker2014domain, FENG2023102664}. However, domain adaptation poses unique challenges due to the sensitive and complex nature of healthcare data \cite{azad2022medical}. The most common associated issues are the limited availability of labeled medical data for training, heterogeneity in data sources contributing to significant domain shifts, clinical disparities and population variances, and inter-rater variabilities. Also, biases present in the source domain data can propagate to the target domain, so ensuring fair and unbiased predictions across diverse patient populations becomes a critical concern. Moreover, medical data encompasses various modalities, including imaging, electronic health records, and genomic data, making the task of adapting models to handle multimodal data and ensuring interoperability exceptionally complex.

Continual learning (CL) - continuous adaptation to new information, has emerged as an important dimension in enhancing the performance and reliability of medical image analysis systems. Transfer learning is widely adopted in the medical domain to address challenges related to limited data availability \cite{YU, Gha}. It transfers knowledge gained from the source task to the target task to improve its learning or performance. The focus is on leveraging prior knowledge rather than retaining it. Unlike transfer learning, CL focuses on both the source domain and the target domain. A CL aims to retain knowledge from previously seen tasks while adapting to new tasks and avoiding catastrophic forgetting issues. CL models are employed for predictive analytics, especially in situations where clinical outcomes can be automatically obtained and incorporated into the algorithm. This capability enhances the model's predictive power by learning from real-time patient data. CL methods can also be employed to utilize the multi-modality dataset for better interpretability and analysis. In recent years, an increasing number of CL methods have been explored and proposed in various subareas of computer vision tasks. \refx{fig:pipeline} presents the paper distributions based on different aspects of CL and shows the growth in exploration in this domain through the rising number of publications over the years. In this paper, we discuss the various aspects of CL, particularly considering its application and implications in the medical domain. Here, we aim to contribute to the ongoing discourse on adapting and improving machine learning models for sustained effectiveness in the dynamic healthcare landscape. By emphasizing CL, we recommend models that not only demonstrate robust performance initially but also possess the ability to evolve and improve over time. CL in medical image analysis represents a powerful approach to developing intelligent systems that can evolve, learn, and adapt to the complexities of healthcare, ultimately contributing to improved patient outcomes and enhanced clinical decision-making. We discuss the limitations and challenges of the existing methods and explore the methods/techniques that can be utilized for developing a robust algorithm. A thorough search of the existing body of literature reveals the groundbreaking nature of our work as the first comprehensive survey of CL techniques applied to medical image analysis. This scholarly endeavor aims not only to contribute novel insights but also to establish a foundational reference for researchers, offering a roadmap that can guide future exploration and incite scholarly interest in the academic community. The primary contributions of our academic pursuit are elucidated below:

$\bullet$~Pioneering in its scope, this survey paper provides the first comprehensive exploration of CL applications in the field of medical image analysis. Our focus extends to delivering a thorough overview encompassing all pertinent papers and elucidating details regarding well-known methods in medical image analysis.

$\bullet$~We introduce a rigorous categorization of CL models within the academic community, presenting a systematic taxonomy that categorizes research based on different CL strategies. Our classification discerns between various CL techniques, such as rehearsal, regularization, architectural, and hybrid methods. Additionally, we contextualize these techniques within various medical sub-fields, offering a nuanced academic perspective.

$\bullet$~Beyond application-centric discussions, our exploration delves into the scholarly challenges and open issues surrounding CL in medical image analysis. By addressing academic intricacies, including data annotation costs, temporal drift, and the necessity for benchmarking datasets, we contribute to the scholarly discourse. Additionally, we identify emerging academic trends that give rise to open questions, shaping the trajectory of future academic research in CL applied to medical image analysis.


\subsection*{Motivation and Uniqueness of this Survey}
\noindent
Over the past few decades, CL approaches in computer vision tasks have seen substantial progress, leading to numerous survey papers exploring deep CL models for computer vision tasks \cite{qu2021recent,wang2023comprehensive,de2021continual,mai2022online}. While some of these surveys focus on specific applications, such as classifications~\cite{de2021continual}, others take a more general approach to concepts and practical perspectives \cite{wang2023comprehensive}. Notably, none of these surveys specifically addresses the applications of CL techniques in medical image analysis, leaving a significant gap in the literature. We believe that insights from successful CL models in vision can be beneficial for the medical community, guiding the retrospective analysis of past and future research directions in CL \cite{verma2023privacy,lee2020clinical}.
CL has proven its potential in developing unified and sustainable deep models capable of handling new classes, tasks, and the evolving nature of data in non-stationary environments across various application areas. Our survey aims to bridge the gap by providing valuable insights that can assist medical researchers, including radiologists, in adopting up-to-date methodologies in their fields. In our survey, we analyze various sources of drifts in medical data, defining CL scenarios in medical images. We present a multi-perspective view of CL by categorizing techniques into rehearsal, regularization, architectural, and hybrid strategies-based methods. The discussion extends beyond applications, encompassing underlying working principles, challenges, and the imaging modality of the proposed methods. We emphasize how this additional information can aid researchers in consolidating literature across the spectrum. A concise overview of our paper is illustrated in \refx{fig:CLtaxonomy}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Search strategy
\subsection*{Search strategy}
\noindent 
\label{sec:search-strategy}
To conduct a thorough literature search, we followed the same strategy presented in \tabrefcite{azad2023advances,azad2023foundational} and utilized DBLP, Google Scholar, and Arxiv Sanity Preserver, employing custom search queries to retrieve scholarly publications related to our topic-CL. 
Our search query was\texttt{
    (continual learning | medical | sequence of tasks) 
    (segmentation | classification | medical | lifelong learning)}.
These platforms allowed us to filter results into categories such as peer-reviewed journal papers, conference or workshop proceedings, non-peer-reviewed papers, and preprints. We carefully filtered our search results through a two-step process: initial screening based on the title and abstract, followed by a subsequent screening of the full text. This approach was instrumental in eliminating false positives, ensuring that only relevant content was included in our study.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Paper organization
\subsection*{Paper organization}\label{sec:paper-organization}
\noindent
All the abbreviations used in this manuscript along with their expansion are tabulated in \refx{tab:fullform}.
A background about various sources of drift in medical data, the catastrophic forgetting issue, CL, a pipeline for CL framework, and CL applications is provided in \refx{sec:background}. Then a thorough description of various kinds of continual learning scenarios found in the medical domain is elaborated in \refx{sec:CLscenario}. Further, we cover various categories of continual learning techniques and their applicability in the medical domain via \refx{sec:CLtechnique}. \refx{sec:CLsupervision} provides details about the level of supervision required in different kinds of proposed frameworks. \refx{sec:evaluation} provides comprehensive practical information such as the experimental setups, training process, and evaluation metrics for measuring the plasticity and stability of continual learning frameworks. \refx{sec:futureDirection} discusses the current challenges in the continual learning literature and future directions. Eventually, the last section provides the conclusion of the survey.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%===================================
\input{content/tables/abbreviations}
%===================================

==> extra/authors/mia.tex <==

\author[1]{Pratibha \snm{Kumari}}
\author[2,3]{Joohi \snm{Chauhan}}
\author[1]{Afshin \snm{Bozorgpour}}
\author[1]{Boqiang \snm{Huang}}
\author[1,4]{Reza \snm{Azad}}
\author[1,5]{Dorit \snm{Merhof}\corref{cor1}}


\cortext[cor1]{Corresponding author: Dorit Merhof, \textit{Tel}.: +49 941 943-68509, \textit{e-mail}: \href{mailto:dorit.merhof@ur.de}{dorit.merhof@ur.de}}

% \ead{dorit.merhof@ur.de}
% \cortext[cor1]{Corresponding author:
% Tel.: +49-241-80-27860}

\address[1]{Faculty of Informatics and Data Science, University of Regensburg, Regensburg 93053, Germany}
\address[2]{University of California, Davis, CA 95616, USA}
\address[3]{Motilal Nehru National Institute of Technology Allahabad, Prayagraj, 211004, India}
\address[4]{Faculty of Electrical Engineering and Information Technology, RWTH Aachen University, Aachen 52062, Germany}
\address[5]{Fraunhofer Institute for Digital Medicine MEVIS, Bremen 28359, Germany}

% \fnref{fn1}
% \fntext[fn1]{This is author footnote for second author.}

% \author[2]{Given-name3 \snm{Surname3}}
%% Third author's email
% \ead{author3@author.com}

==> extra/keywords/mia.tex <==

Continual Learning\sep
Medical Data Drift\sep
Domain Shift\sep
Concept Drift\sep
Medical Image Analysis\sep
Histopathology\sep
Radiology
